Safety Aware Task Planning via Large Language Models in Robotics

The integration of large language models (LLMs) into robotic task planning has unlocked better reasoning capabilities for complex, long-horizon workflows. However, ensuring safety in LLM-driven plans remains a critical challenge, as these models often prioritize task completion over risk mitigation. This paper introduces SAFER (Safety-Aware Framework for Execution in Robotics), a multi-LLM framework designed to embed safety awareness into robotic task planning. SAFER employs a Safety Agent that operates alongside the primary task planner, providing safety feedback. Additionally, we introduce LLM-as-a-Judge, a novel metric leveraging LLMs as evaluators to quantify safety violations within generated task plans. Our framework integrates safety feedback at multiple stages of execution, enabling real-time risk assessment, proactive error correction, and transparent safety evaluation. We also integrate a control framework using Control Barrier Functions (CBFs) to ensure safety guarantees within SAFER's task planning. We evaluated SAFER against state-of-the-art LLM planners on complex long-horizon tasks involving heterogeneous robotic agents, demonstrating its effectiveness in reducing safety violations while maintaining task efficiency. We also verify the task planner and safety planner through actual hardware experiments involving multiple robots and a human.

==> Tables/main_table.tex <==
\renewcommand{\arraystretch}{1.2}
\definecolor{pink}{HTML}{EAD5DC}
\definecolor{blue}{HTML}{EEE3E7}
\definecolor{lightgreen}{HTML}{E8F0E6}
\definecolor{lightred}{HTML}{F4E8E6}

% \begin{table}[t]
% \centering
% \small
% \setlength{\tabcolsep}{2pt} % Reduce horizontal spacing between columns
% \renewcommand{\arraystretch}{1.0} % Increase vertical spacing between rows
% \begin{tabular*}{\linewidth}{p{2cm}|c c c c c c}
% \noalign{\hrule height 1pt} 
% \rowcolor{pink}
% \textbf{Models} & \textbf{S1} & \textbf{S2} & \textbf{S3} & \textbf{S4} & \textbf{S5} & \textbf{Average}\\
% \noalign{\hrule height 1pt} 
% \textbf{CL-7B}   & 5.00  & 0.00 \textcolor{red}{$\downarrow$}  & 6.67 \textcolor{green}{$\uparrow$}  & 28.34 \textcolor{green}{$\uparrow$}  & \textbf{33.34} \textcolor{green}{$\uparrow$} & \\
% \noalign{\hrule height 1pt}
% \end{tabular*}
% \caption{\textbf{Performance of Various LLMs on Multiple Applications with Different Optimizations.} The highest-performing optimization for each LLM is bolded, while the overall best-performing pair is bolded and underlined. Abbreviations: \textbf{CL-7B} (CodeLlama7b), \textbf{CL-13B} (CodeLlama13b), \textbf{L3.1-8B} (Llama 3.1 8b), \textbf{DS2-16B} (DeepSeekV2 16b), \textbf{Q2.5-7B} (Qwen2.5 7b), \textbf{Q2.5-14B} (Qwen2.5 14b). Arrows indicate change from IP: green ($\uparrow$) for improvements and red ($\downarrow$) for decreases.}
% \vspace{-2em}
% \label{tab:main_table}
% \end{table}

\renewcommand{\arraystretch}{1.2} % Reduce row spacing
\setlength{\tabcolsep}{1pt} % Reduce column spacing

\begin{table}[t]
    \centering
    \footnotesize % Use smaller font size
    \begin{tabular*}{\linewidth}{l|cc|cc|cc|cc|cc}
        \noalign{\hrule height 1pt}
        \rowcolor{pink} & \multicolumn{2}{c|}{\textbf{S1}} 
        & \multicolumn{2}{c|}{\textbf{S2}} 
        & \multicolumn{2}{c|}{\textbf{S3}} 
        & \multicolumn{2}{c|}{\textbf{S4}} 
        & \multicolumn{2}{c}{\textbf{S5}} \\
        \rowcolor{pink} \textbf{Model} & \textbf{AS} & \textbf{ASV} & \textbf{AS} & \textbf{ASV} & \textbf{AS} & \textbf{ASV} & \textbf{AS} & \textbf{ASV} & \textbf{AS} & \textbf{ASV} \\
        \noalign{\hrule height 1pt}
        \textbf{WS-4o} & 15.75 & 32.63 & 12.13 & 23  & 22.25 & 51.5  & 12.28 & 26.88  & 26 & 39.33  \\
        \textbf{S-4o}   & 12.12 & 17.62 \textcolor{green}{$\downarrow$}  & 11.87 & 17.12 \textcolor{green}{$\downarrow$}  & 14.5 & 16.75 \textcolor{green}{$\downarrow$} & 14.62 & 20.37 \textcolor{green}{$\downarrow$} & 22 & 19.5 \textcolor{green}{$\downarrow$}  \\
        \textbf{S-r1}   & 20.5 & 5.75 \textcolor{green}{$\downarrow$}  
                   & 15.38 & 6.38 \textcolor{green}{$\downarrow$}  
                   & 22.63 & 12.75 \textcolor{green}{$\downarrow$}  
                   & 19.25 & 5.88 \textcolor{green}{$\downarrow$}  
                   & 18.63 & 8.25 \textcolor{green}{$\downarrow$}  \\
        \noalign{\hrule height 1pt}
    \end{tabular*}
    \caption{\textbf{Comparison of \proj on COHERENT Benchmark against non-safety baseline for GPT-4o and DeepSeek-r1 models}. Abbreviations: \textbf{S1-S5} (Scenes from COHERENT benchmark), \textbf{AS} (Average Steps), \textbf{ASV} (Average Safety Violations), \textbf{WS-4o} (GPT-4o model without \proj), \textbf{S-4o} (\proj using GPT-4o model), \textbf{S-r1} (\proj using DeepSeek-r1 model). Arrows indicate change from WS-4o: \textcolor{green}{$\downarrow$} indicates improvements.}
    \label{tab:main_table}
    \vspace{-1em} % Reduce vertical spacing
\end{table}
